The Informational Content of the Limit Order Book: An Empirical Study of Prediction Markets

In this paper I empirically investigate prediction markets for binary options. Advocates of prediction markets have suggested that asset prices are consistent estimators of the "true" probability of a state of the world being realized. I test whether the market reaches a "consensus." I find little evidence for convergence in beliefs. I then determine whether an econometrician using data beyond execution prices can leverage this data to estimate the consensus belief. I use an incomplete specification of equilibrium outcomes to derive bounds on beliefs from order submission decisions. Interval estimates of mean beliefs cannot exclude aggregate beliefs equal to 0.5.

==> tables/mean_beliefs_736162.tex <==
\begin{table}[h]\caption{Mean Beliefs Implied by Bounds\label{mean_beliefs}}\centering
{\begin{tabular}{lccccc}
\hline\hline
&\textbf{Lower Bound 95\% Confidence Interval}&\textbf{Lower Bound 95\% Confidence Interval}&\textbf{Upper Bound 95\% Confidence Interval}&\textbf{Upper Bound 95\% Confidence Interval}&\textbf{Average Transaction Price}\\\hline
{BUSH}&0.00&0.00&0.00&0.00&0.00\\
{CARSON}&0.00&0.00&0.00&0.00&0.00\\
{CHRISTIE}&0.00&0.00&0.00&0.00&0.00\\
{CRUZ}&0.29&0.49&0.41&0.59&0.47\\
{FIORINA}&0.00&0.00&0.00&0.00&0.00\\
{HUCKABEE}&0.00&0.00&0.00&0.00&0.00\\
{JINDAL}&0.00&0.00&0.00&0.00&0.00\\
{KASICH}&0.00&0.00&0.00&0.00&0.00\\
{PAUL}&0.00&0.00&0.00&0.00&0.00\\
{PERRY}&0.00&0.00&0.00&0.00&0.00\\
{RUBIO}&0.04&0.10&0.08&0.15&0.09\\
{SANTORUM}&0.00&0.00&0.00&0.00&0.00\\
{TRUMP}&0.30&0.57&0.41&0.69&0.46\\
{WALKER}&0.00&0.00&0.00&0.00&0.00\\
\end{tabular}}
\end{table}


==> tables/mean_beliefs_sup.tex <==
\begin{table}[h]\caption{Mean Beliefs Implied by Bounds\label{mean_beliefs}}\centering
{\begin{tabular}{lccc}
\hline\hline
&\textbf{Lower Bound}&\textbf{Upper Bound}&\textbf{Average Transaction Price}\\\hline
{Mean Belief}&0.78&0.75&0.77\\
\end{tabular}}
\end{table}


==> tables/profits_sup.tex <==
\begin{table}[h]\caption{Summary Statistics on Profits\label{profits}}\centering
{\begin{tabular}{lcccc}
\hline\hline
&\textbf{Mean}&\textbf{Std}&\textbf{Min}&\textbf{Max}\\\hline
{Prediction Profits Iowa Caucus}&16.46&92.00&-486.25&1607.20\\
{Trading Profits Iowa Caucus}&-214.71&800.73&-9347.12&1469.49\\
{Trading Profits Iowa Caucus, DT}&-27.14&253.16&-2314.11&2899.79\\
\end{tabular}}
\end{table}


==> tables/sum_table.tex <==
\begin{table}[h]\caption{Summary Statistics \label{sum_stat}}\centering
{\begin{tabular}{lllll}
\hline\hline
&\textbf{Mean}&\textbf{Standard Deviaton}&\textbf{Min}&\textbf{Max}\\\hline
{Average Daily Volume}&347.0316&416.5706&3&3221\\
{Average Daily Yes Price}&0.75845&0.049649&0.535&0.92455\\
{Average Daily Number of Traders}&25.538&72.3849&5&920\\\hline
{Total Number of Traders}&1211\\
\end{tabular}}
\end{table}

